Calibrating Predictions to Decisions: A Novel Approach to Multi-Class Calibration

When facing uncertainty, decision-makers want predictions they can trust. A machine learning provider can convey confidence to decision-makers by guaranteeing their predictions are distribution calibrated -- amongst the inputs that receive a predicted class probabilities vector $q$, the actual distribution over classes is $q$. For multi-class prediction problems, however, achieving distribution calibration tends to be infeasible, requiring sample complexity exponential in the number of classes $C$. In this work, we introduce a new notion -- \emph{decision calibration} -- that requires the predicted distribution and true distribution to be ``indistinguishable'' to a set of downstream decision-makers. When all possible decision makers are under consideration, decision calibration is the same as distribution calibration. However, when we only consider decision makers choosing between a bounded number of actions (e.g. polynomial in $C$), our main result shows that decisions calibration becomes feasible -- we design a recalibration algorithm that requires sample complexity polynomial in the number of actions and the number of classes. We validate our recalibration algorithm empirically: compared to existing methods, decision calibration improves decision-making on skin lesion and ImageNet classification with modern neural network predictors.

==> desiderata.tex <==
\subsection{Desiderata of Uncertainty for Decision Making}

%This is useful because the forecaster usually have some prior knowledge that most decision makers who use the prediction function , and can guarantee the desirable properties $\hp$ for any loss function $\ell \in \Lc$. 


\paragraph{Accurate loss estimation.} First and foremost, a decision maker want assurance that making decisions based on a prediction function $\hp$ give low expected loss. %At the very least she should know whether the decisions will give low expected loss or not. 
Suppose the decision maker uses the Bayes decision rule $\delta_\ell$ (as in Definition~\ref{def:bayes_decision}), then without knowing the outcome $Y$, she can compute her ``simulated'' loss: 
$
\Eb_X \Eb_{\aY \sim \hp(X)} [\ell(\aY, \delta_{\ell}(\hp(X))) ] 
$. This is the loss a decision maker expects to incur assuming the predictions are correct, i.e. the outcome $Y$ indeed is drawn from the predicted distribution $\hp(X)$. To assure decision makers that she will not incur any additional loss in surprise, the ``simulated'' loss should equal the true loss. 

% In particular, we want the predicted loss to be indicative of the actual decision loss, which we formalize as the following 

Formally, a prediction function $\hp$ satisfies accurate loss estimation (with respect to $\Lc \subset \Lall$ and $p^*$) if $\forall \ell \in \Lc$ 
\begin{align}
    \Eb_X \Eb_{\aY \sim \hp(X)} [\ell(\aY, \delta_{\ell}(\hp(X))) ] = \Eb_X \Eb_{Y \sim p^*(X)} [\ell(Y, \delta_{\ell}(\hp(X))) ] \label{eq:accurate_loss}
\end{align}
For example, given Eq.(\ref{eq:accurate_loss}), a hospital can test the prediction function $\hp$ on the features of its current patients; if the simulated loss is small, then the hospital will know that using $\hp$ and the Bayes decision rule $\delta_\ell$ leads to low expected loss. If the simulated loss is large the hospital can look for alternative solutions. 

%s If the simulated loss is already very large, then the decision maker will want to consider a different predictor, 
% Intuitively, the left hand side of Eq.(\ref{eq:accurate_loss}) is the expected loss of the decision making assuming that the predictions are correct (i.e. the label $\aY$ is drawn from the predicted distribution $\hp(X)$; the right hand side is the true loss of the decision maker (where the label $Y$ is drawn from $p^*(X)$). 

\paragraph{Strategyproofness.} % the prediction function should discourage any strategic mis-specification of the loss function. 
%encourage the decision maker to come up with the correct loss function. \se{what does this mean? are we now assuming the decsion maker picks the loss after seeing the forecaster?}
Another property we consider is that that the prediction should discourage intentional mis-specifying the loss function. For example, without guarantees on the predicted probabilities, a hospital may need to be strategic in their recommendation of treatments. For example, hospitals may worry that the predicted probability of a severely bad outcomes (if left untreated) is lower than reality. The hospital might artificially modify its loss function so that the (modified) optimal decision rule recommends invasive treatments more often. This strategy would hedge against costly false negatives, but comes with the risks associated with over-diagnosis and  over-treatment~\citep{esserman2013overdiagnosis}. 

The decision maker only has to concerned about specifying her true preferences as accurately as possible, and does not have be concerned about the interplay between the loss function and the prediction function. 

%achieve smaller loss than the Bayes decision rule that corresponds to any other loss function. 
Formally, a prediction $\hp$ is strategy proof (with respect to $\Lc \subset \Lall$ and $p^*$) if $\forall \ell, \ell' \in \Lc$ 
\begin{align}
    \Eb[\ell(X, Y, \delta_\ell(\hp(X)))] \leq  \Eb[\ell(X, Y, \delta_{\ell'}(\hp(X)))] \label{eq:truth_rewarding}
\end{align}
%In other words, a  $\hp$ encourages a decision maker to accurately specify her true loss function, because she 
In other words, a decision maker cannot do better by choosing an inaccurate loss function that does not reflect her true preferences. 

==> intro.tex <==

% \begin{enumerate}
%     \item Decision makers (hospitals) use predicted probability to make decisions, but don't have enough data / expertise to learn their own prediction function, so want to use a third party prediction service. 
%     \item But how can the decision maker know the third party prediction service is good? One option is to try its patient's unlabeled data and obtain probability predictions. If the probabilities are accurate, then the hospital can assess their expected loss if they use the prediction service to make decisions. For example, if the prediction service is highly unconfident and return the marginal probability on all patients, then hospital 
% \end{enumerate}

% Machine learning is commonly used when making high-stakes decisions.
% Consider a hospital that wants to diagnose skin lesions, in order to recommend appropriate treatment.
% The hospital may know the various possible skin conditions (classes), the available treatments (actions), and the likely health outcome (loss) incurred under each treatment for each given condition.
% To aid in diagnosis, the hospital could use a supervised learning model that, given an image of the lesion, predicts the probability of each condition.
% If the predicted probabilities were correct, then the hospital could simply choose the treatment that optimizes the patient's outcome (i.e., minimizes their expected loss) to obtain an effective decision rule.
% The typical hospital, however, does not have the data or computational resources necessary to train a sophisticated predictor on their own. \se{logic is a bit unclear. seem to conflate having exact probabilities vs end-to-end training on a specific loss function}
% \mpk{this is a good point. maybe need to start with perspective of ML provider. emphasize that hospitals may be distrustful because they have varied losses, and provider may be selling the same model to all of them. we show a sense in which this is possible for both provider and hospitals.}
% In this case, they  may consider purchasing a pre-trained model from a machine learning service.
% While convenient, outsourcing the training to a third party raises two key issues of trust:
Machine learning is commonly used when making high-stakes decisions.
Consider a setting where a machine learning provider contracts with hospitals that want to diagnose skin lesions in order to recommend appropriate treatment.
Each hospital knows the various possible skin conditions (classes), the treatments available on site (actions), and the likely health outcomes (loss) incurred by patients in their population under each treatment for each condition.
To aid in diagnosis, ML service can develop a supervised learning model that, given an image of the lesion, predicts the probability of each condition.
If the predicted probabilities were correct, then the hospitals could simply choose the treatment that optimizes their patients' outcomes (i.e., minimizes their expected loss) to obtain an effective decision rule.
While purchasing a pre-trained model may be convenient, outsourcing the training to a third party raises two key issues of trust for the hospitals:
\begin{itemize}
    \item First and foremost, each hospital may want assurance that the model's predictions lead to beneficial decisions, according to their own loss function.
    % Understanding the consequences of using the prediction function is essential for ensuring reliable treatment.
    Concretely, the hospitals may reasonably worry that the model was trained using a loss function different than their own.
    This mismatch is often inevitable because the ML service may provide the same prediction model to many hospitals, which may have different loss functions.
    Even the same hospital could have different loss functions throughout time, due to changes in treatment availability. %It would be prohibitively expensive for a machine learning service to optimize a new prediction model for each possible loss functions. %a might provide the same prediction model to multiple hospitals with different loss functions; even for the same hospital .  
    %\se{can also say that if the same ml service provides same  predictions to multiple users with different losses, mismatch is inevitable}
    
    \item Second, without guarantees on the predicted probabilities, the hospitals may need to be strategic in their recommendation of treatments.
    For example, hospitals may worry that the predicted probability of melanoma---which leads to severely bad outcomes if left untreated---is lower than reality.
    % , which causes insufficient invasive treatments.
    The hospital might artificially 
    modify their loss function so that the (modified) optimal decision rule
    % that minimizes the modified loss function 
    %in order to 
    recommends invasive treatments more often.
    %\se{need to justify why changing the loss modifies the actions}
    This strategy would hedge against costly false negatives, but comes with the risks associated with over-diagnosis and  over-treatment~\citep{esserman2013overdiagnosis}.
\end{itemize}





To address these two concerns, the hospitals may insist that the prediction function be \emph{calibrated}.
Calibration guarantees that the predictions define a valid probability model that plausibly could generate the data distribution.
% Formally, for a multi-class task with $C$ different classes, a prediction function $\hp:\Xc \to \Delta^C$ maps individuals $x \in \Xc$ to a discrete probability distribution $q \in \Delta^C$ over the classes; we say that $\hp$ is \emph{distribution calibrated} if for all $q \in \Delta^C$,
% \begin{align*}
%     Y \mid \hp(X) = q \text{ has distribution } q
% \end{align*}
% \se{not a fan of math in the intro. formulas ends up being confusing because symbols are not yet defined}\sj{I tried some lightening of the notation}\mpk{I like this less. we can rework to use less math.} 
More formally, for a multi-class task with $C$ different classes, a predictor $\hp$ maps individuals $x$ to a discrete probability distribution over the classes $\hp(x)$.
We say that $\hp$ is \emph{distribution calibrated} if, averaged over the individuals $x$ who receive predicted distribution $\hp(x) = q$, the true distribution over classes is $q$.
In this way, distribution calibration addresses the two key concerns: to start, the decision-maker can understand the consequence of using the prediction function because among the patients who receive prediction $q$, the hospitals knows their true label distribution (which is also $q$) and hence know the true expected loss of a treatment on these patients;
% second, we will show 
it follows that strategizing can never lead to better treatment decisions, so should be out of consideration for the hospitals.
% \mpk{I don't think this is novel. Isn't this the point of these strictly proper scoring rules?  Fine to say, I would just remove ``we will show''}
% imagine that the outcomes are distributed $\hat{Y} \sim \hp(X)$ according to the predictions, and calculate the expected loss and optimal action (without strategizing) accordingly. \se{unclear why this is the case}

% \mpk{TODO:  need to argue distribution calibration is sufficient.}



% On the one hand, distribution calibration is quite easy to achieve on its own: the learner can simply output $\bar{q}$ for all $x \in \Xc$, where for each class $c \in [C]$, $\bar{q}_c = \Pr[Y = c]$ represents the marginal probability for the class.
% On the other hand, this marginal predictor is useless (indeed, it is constant across $\Xc$).

Unfortunately, effective methods for establishing distribution calibration have remained elusive.
To achieve distribution calibration, we need to reason about the set of individuals $x$ who receive prediction $\hp(x) = q$ for each $q$ 
%reason about every possible predicted distribution 
%that is supported by 
in the support of the predictor.
As the size of the support may naturally grow exponentially in the number of classes $C$, the amount of data needed to accurately certify distribution calibration tends to be prohibitive.
% For even modestly sized classes ($C \ge 10$),
% \todo{Shengjia, is this true? Also, let's find references we can use to back up the many efforts and difficulty of calibration.\sj{I don't think there is a good reference for this, the papers that propose distribution calibration certainly will not spend effort saying it's really hard :) } },
% \se{feels a bit too detailed for an intro. can probably just state as a fact, and justify later in main paper}
Due to this statistical barrier, most work on obtaining calibrated multi-class predictions focuses on obtaining relaxed variants of calibration.
These include \emph{confidence calibration} \citep{guo2017calibration}, which calibrates predictions only over the most likely class, and \emph{classwise calibration} \citep{kull2019beyond}, which calibrates predictions for each class marginally.
While feasible, intuitively, these notions are significantly weaker than distribution calibration.
In particular, we show that these relaxations do not address either of the two trust issues highlighted above. %\se{can claim this observation as a contribution?}


%\se{there should be a crisp 1 sentence problem statement somewhere. "designing training objectives/recalibration so that output probabilities can be used to reliably estimate expectations/loss by downstream decision-makers"}

Is there a notion of calibration that addresses both issues of trust, but can also be verified and achieved efficiently? Our paper answers this question affirmatively. 

\paragraph{Our Contributions.} 
%Distribution calibration addresses the issues of trust, but is difficult to verify or achieve; weaker calibration notions do not address the trust issues. 
%We revisit the problem of obtaining calibrated predictors from a decision-making perspective. 
% We introduce a new notion of calibration---\emph{decision calibration}---where, intuitively, we calibrate predictions, not according to the predicted value, but according to the downstream decision that results from the prediction.



% We introduce a new notion of calibration---\emph{decision calibration}---where, intuitively, we calibrate predictions to downstream decisions rather than to the predicted values.
% In other words, from the perspective of a decision-maker, a set of decision calibrated predictions should be
% practically \emph{indistinguishable} from the true probability distribution over classes.
% \mpk{Let's be more specific.  rather than ``indistinguishable'' say that any loss from the class, under any decision rule from the class is accurate?}
% For example, to a decision-maker whose loss is identical under outcome A and outcome B, a prediction function should be indistinguishable from the true probability if its only prediction mistakes are between outcome A and outcome B. \mpk{Not sure I understand.}
% We show that indistinguishability naturally implies the two notions of trust highlighted above.
% Our study of decision calibration yields new insights---both conceptual and practical---about obtaining calibrated predictions.
%% michael's edits
We introduce a new notion of calibration---\emph{decision calibration}---where
%, intuitively, we calibrate predictions to downstream decisions rather than to the predicted values.
%Decision calibration  \sj{I feel like the previous sentence was less understandable than the following sentence}
we take the perspective of potential decision-makers:  the only differences in predictions that matter are those that could lead to different decisions.
Inspired by \citep{dwork2021outcome}, we formalize this intuition by requiring that predictions are ``indistinguishable'' from the true outcomes, according to a collection of decision-makers.
In more detail, %decision calibration %considers the distribution over outcomes defined by the predictor and compares it to the true distribution over outcomes. \sj}I feel like this sentence is redundant} 
given a collection of loss functions and decision rules, a predictor is decision calibrated with respect to the collection, if for each loss and decision rule, the expected loss using the decision rule is the same under the predicted and true distributions.
Our study of decision calibration yields new insights---both conceptual and practical---about obtaining calibrated predictions.



First, we show that all prior notions of calibration can be characterized as variants of decision calibration under different decision-makers.
This framing explains the strengths and weakness of existing notions of calibration.
% For example, distribution calibration is the necessary and sufficient condition for indistinguishability under \textit{all} decision tasks. 
For example, we show that a predictor is distribution calibrated if and only if it is decision calibrated with respect to \emph{all} loss functions and decision rules. %  over an action space that grows linearly in the support size of the predictor. \sj{We haven't mentioned action space before, so this could be a bit confusing} 
This characterization demonstrates why distribution calibration is so challenging: achieving distribution calibration requires simultaneously reasoning about all possible decision tasks. 
Additionally, we show that the existing relaxed notions of calibration correspond to decision calibration with respect to very simple, restricted sets of decision tasks.
This result clarifies the limitations of the relaxations of calibration: the relaxed notions provide guarantees for sets of decision tasks that are very limited, and unlikely to apply to realistic decision-makers.
\sj{I'm a little concerned about the transition from loss functions and decision rules to decision tasks, but maybe that is okay} 
% Instead of calibrating to all decision tasks, the machine learning service can calibrate to a carefully selected set of decision tasks, and declare this selection to downstream decision makers. Consequently a decision maker can check if her decision task belongs to the advertised set, and trust the prediction function whenever this is the case. We show that existing relaxed notions of calibration correspond to calibration to very simple, restricted sets of decision tasks.

% This framing explains the weakness of the relaxed notions of calibration, which 

% However, not all decision tasks are created equal, and many decision tasks rarely arise in practice. For example, it is unlikely that a healthcare provider will have to decide between $2^{100}$ distinct treatment options.

Distribution calibration can guarantee decision calibration with respect to decision rules that choose between exponentially (in number of classes $C$) many actions. 
%Note that the characterization of distribution calibration requires an action space that grows, possibly exponentially in the number of classes $C$.
In practice, however, decision-makers typically choose from a bounded (or slowly-growing as a function of $C$) set of actions.
% In most realistic applications, it is safe to assume that the number of possible actions is reasonably bounded.
Our main contribution is an algorithm that \textbf{guarantees %a strong variant of 
decision calibration for such realistic decision-makers}.
% Our key result is that it is feasible to calibrate to almost all realistic decision tasks. 
%We show that %whenever decision-makers have a bounded number of possible actions, 
%we can efficiently achieve decision calibration---.
In particular, we give a sample-efficient algorithm that takes a pre-trained predictor and post-processes it to achieve decision calibration with respect to \emph{all} decision-makers choosing from a bounded set of actions. %over the bounded action space.
Our recalibration procedure does not harm other performance metrics, and slightly improves accuracy and likelihood of the predictions. 
%Unlike the trivial approaches to achieve calibration---which destroy information---our recalibration procedure improves the likelihood of the underlying predictions.
%Importantly, t

Our recalibration algorithms outputs predictors that address the two key reliability concerns from above, allowing for accurate loss estimation and strategyproof decision-making. Empirically, we use our algorithm to recalibrate deep network predictors on two large scale datasets: skin lesion classification (HAM10000) and Imagenet. Our recalibration algorithm improves decision making, and allow for significantly more accurate loss estimation compared to existing recalibration methods. %Figure~\ref{fig:ham} shows an example where a confidence calibrated prediction function breaks the first reliability concern of accurate loss estimation, while our recalibration algorithm corrects  

% \sj{I feel like the following argument is too delicate, maybe we should consider not mentioning it in the intro?}
% \mpk{Fine by me, but let's discuss.}
% In fact, we show that the post-processed predictions are approximately distribution calibrated.
% This surprising result follows from a key insight: if there are a bounded number of possible actions, then the salient information can be ``compressed'' into a bounded support calibrated predictor, without incurring additional loss.
% In other words, we can effectively sidestep the statistical roadblocks to distribution calibration, without reducing the informativeness of the predictions.
%In all, we give a principled and effective approach for obtaining a strong notion of calibration for multi-class predictors.
    

% %, we calibrate predictions to the downstream decisions, rather than to the predicted value. 
% \se{this part should be significantly expanded. shorten background to bare minimum, and use more space to explain your contribution}

% Studying decision calibration yields new insights---both conceptual and practical---in obtaining calibrated predictions.
% \begin{itemize}
%     \item 

%     \item

% \end{itemize}
% 




% \mpk{end of my intro.}




% Outline:
% \begin{itemize}
%     \item Two key desiderata:
%     \begin{itemize}
%         \item Accurate loss estimation:  whatever the decision-maker's loss $\ell$, the expected loss should be reflected by imagining $\hat{Y} \sim \hp$.
%         \item Strategyproof decision-making:  whatever the decision-maker's loss $\ell$, they should be able to choose the best action by choosing the optimal action as if $\hat{Y} \sim \hp$, i.e., $\delta_\ell(\hp(X))$
%         \item Given $\hp$, the only ``decision'' the decision-maker needs to make is whether their estimated expected loss is acceptable or not: if so, simply use the optimal decision rule $\delta_\ell(\hp(X))$, and the expected loss will be obtained; if not, then reject the predictor $\hp$ and ask for a better one.
%     \end{itemize}
%     \item How to achieve?
%     \begin{itemize}
%         \item (Distribution) Calibration: can imagine that $\hp$ defines the parameters of a probabilistic model that generates the data
%         \item This perspective immediately gives the two desiderata
%     \end{itemize}
%     \item Problem:
%     \begin{itemize}
%         \item Effective methods for establishing distribution calibration for informative predictors has remained elusive.
%         \item Could always take the marginal predictor, but doesn't give any information
%         \item If we have an informative predictor $\hp$, in general, can't even certify that it satisfies distribution calibration.
%         \item Sample complexity needed to certify scales linearly in the size of the support of $\hp$; for informative predictors, size of support reasonably may grow exponentially in the number of classes
%     \end{itemize}
%     \item Existing relaxations: to get at feasible notions, focus has been on relaxations
%     \begin{itemize}
%         \item Confidence: condition only on the max prediction
%         \item Classwise: conditioning only on the marginal value of each class
%         \item intuitively, much weaker. cannot guarantee desiderata for arbitary loss functions.
%     \end{itemize}
%     \item Our contributions:
%     \begin{itemize}
%         \item We revisit the problem from a decision-making perspective.  Helps to clarify the existing notions of calibration and make progress on achieving the desiderata.
%         \item Introduce a novel notion of calibration: decision calibration.
%         \item for all $\ell \in \Lc$ and for all $\delta \in \Dc$
%         \begin{align*}
%             \Eb[\ell(\hat{Y}, \delta(\hp(X)))] = \Eb[\ell(Y, \delta(\hp(X)))]
%         \end{align*}
%         \item \mpk{add intuition}
%     \end{itemize}
%     \item Prior notions:
%     \begin{itemize}
%         \item We show all prior notions of calibration can be formulated as variants of decision calibration
%         \item clarifies prior work:
%         \begin{itemize}
%             \item weak notions correspond to highly restricted loss classes and decision rules
%             \item distribution calibration is challenging because it corresponds to reasoning about all losses simultaneously
%             \item these losses are defined over an action space that grows linearly in the support of $\hp$
%         \end{itemize}
%     \end{itemize}
%     \item Reframing the goal: decision-making!
%     \begin{itemize}
%         \item The salient information of any predictor is what you do with the predictions
%         \item in a sense, the sets we care about most are not necessarily the support of $\hp$, but rather the sets defined by decision rules (in particular, optimal decision rules for a rich set of loss functions).
%         \item In particular, if we restrict our attention to decision-makers who have a modest number of possible actions (e.g., growing polynomially in the number of classes), then we may hope to achieve distribution calibration without destroying information in predictions
%         \item Positive result:  show a post-processing algorithm
%         \begin{itemize}
%             \item takes in any predictor
%             \item post-processing can only improve the closeness to the true model of $Y$ \mpk{is there a way to formalize that it's getting closer for all loss functions? or at least on average? or at least for loss functions that are monotone in the likelihood or something?} improves the likelihood of the model.
%             \item achieves decision calibration for all losses!
%             \item we show that this strong notion of decision calibration implies distribution calibration with ``good'' loss \mpk{would love to compare to the loss of the original predictor}
%             \item Of note: algorithm follows by observing a connection to the idea of mutli-calibration, where the important class of ``distinguishers'' is derived from the set of potential optimal decision rules.
%         \end{itemize}
%     \end{itemize}
% \end{itemize}











% \begin{itemize}
%     \item healthcare provider can't train their own model
%     \item Two issues if they outsource:
%     \begin{itemize}
%         \item How do they know how well the predictor will perform (overall)?  For instance, what if they third-party trained the ML model using a loss different than the healthcare provider's?
%         \item Given distrust about the accuracy of individual predictions, how does the healthcare provider select a decision rule?  May need to be strategic, selecting a strategy that hedges against potential inaccuracies.
%     \end{itemize}
% \end{itemize}

% Machine learning is commonly used to make predictions in high-stakes decisions.
%, such as medical treatment recommendation. 
% or autonomous driving.
% Consider a healthcare provider that wishes to use machine learning to diagnose skin lesions in order to recommend appropriate treatment.
% ~\citep{tschandl2018ham10000} %% cite later and
% to aid in diagnosing conditions
% Usually the healthcare provider knows their available treatments and can estimate their loss function (i.e. the loss of applying treatment x if the lesion classification is y, an example loss function is shown in Figure~\ref{fig:ham} left panel).
% The healthcare provider usually knows the possible skin conditions (classes), the available treatments (actions), and the likely health outcome (loss) incurred by each treatment for each given condition.
% If the predicted probabilities of each condition are correct, then the healthcare provider can choose the treatment that optimizes the patient's likely outcome (i.e., minimizes their expected loss).
%For example, a healthcare provider might recommend an invasive surgery if the probability of the skin lesion being malignant is greater than 10\%. 

% However, the healthcare provider typically lack sufficient data to train its own prediction function, and 
%To learn an accurate prediction function the healthcare provider will need a large amount of expensive labeled data. Therefore, each healthcare provider might 
% have to purchase a black box prediction function from a third party provider. In addition, prediction functions are almost never perfect, and inaccurate predictions can lead to poor treatment recommendations.

%A provider might offer a probabilistic diagnosis prediction function to a healthcare provider, a vision company might provide a object classification function to autonomous driving company. 

% How can the healthcare provider trust the third party prediction function? One important element is contractual trust~\citep{jacovi2021formalizing}, where the consequence and potential loss of using the prediction function should be known in advance.
% %To convey confidence to the healthcare provider, the consequence of deploying the prediction function should be known. 
% For example, the healthcare provider might want to try out the prediction function on its patient's features, and compute (before deployment) the expected number of incorrect treatments if the prediction function is deployed. If the healthcare providers computation is guaranteed to be correct, then the benefit or harm of using the prediction function is known in advance. The healthcare provider can then compare the prediction function with offerings from competitors or human experts, and confidently know whether adopting the prediction function benefits patients. 


% Calibration is a method of conveying confidence. In particular, among the patients whose predicted probability of   Say that calibration achieves the above, and sometimes do not. We formalize this intuition as decision calibration. 

% % As a motivating example, consider a skin lesion diagnosis task. Invasive tests such as surgical histology provide the ground truth label, while non-invasive imaging can be used to predict the ground truth label with high but imperfect accuracy. Healthcare providers can use low cost images and a prediction model to predict the ground truth, and refer suspicious cases for invasive tests. For example, the patient might undergo invasive tests if the probability of melanoma is $>$5\%. % or if the probability of (mildly dangerous) basal cell carcinoma is $>$5\%. 


% %If we assume that utility can be measured by monetary units, then an insurance-like mechanism can provide individual level guarantees. However, when measuing utility with monetary units 

% A weaker but achievable requirement is confidence calibration or classwise calibration. 
% %For example, to satisfy classwise calibration, among the patients where the model predicts has 1\% chance of melanoma, indeed 1\% of them have melanoma. 
% However, consider two models A and B that are classwise calibrated: for the patients whom model A or B predicts 5\% chance of melanoma, 5\% of them have melanoma. Among these patients with melanoma, suppose model A assigns 10\% probability to carcinoma, while model B assigns 0 probability to other dangerous conditions. A care provider who uses model A might refer the patient for invasive tests (because of the concern for both melanoma and carcinoma), while model B might not. Model A and B are equally good under the classwise or confidence calibration metric, but model B can lead to poor high risk decisions (at least for the patients with melanoma). 

% We observe in Figure 1, a densenet model trained on HAM10000 behaves like model B in the above example. Among the patients whom the prediction model (incorrectly) assign a low chance of melanoma, almost all of the probability mass is assigned to benign conditions. Given the decision loss function shown in Figure 1 (middle), suppose a health care provider chooses the Bayes action (i.e. the action with minimum expected loss under the \textit{predicted} distribution). If these predicted probability are correct, the expected loss should be -0.14, while based on the ground truth labels the expected loss is actually -0.16. In other words, there is unexpected harm of the patients. Importantly, this unexpected harm might go unnoticed because we only know the ground truth label for patients that actually underwent the invasive test, and do not know the label of patients who didn't.  %In other words, the true loss is larger than the expected 
% \mpk{Let's discuss this figure.  I think it might be a bit distracting for the intro.  There's a lot to unpack technically, and it might distract from the main message.  It's nice that it's real, but in a sense a cartoon might communicate the goal more clearly.}

% This example points to an important element of trust (which (cite) calls as contractual trust), where the true consequence of using the prediction algorithm should be known. In our case, if the loss is predicted to be -0.14, then it should be -0.14 in reality. There should be no additional loss or harm that is unknown when making these decisions. We formalize this desiderata in a definition we call decision calibration. 



% In this paper we identify minimal conditions for making safe decisions --- the expected loss of the decision making agent is the same under the predicted distribution and the true distribution --- which we call decision calibration. We show that decision calibration can be verified and achieved with sample size that is linear in both the set of actions and the number of classification categories. 



% Consider an autonomous driving agent who is trying to decide between one of five actions (e.g. keep going, decelerate, turn left, turn right, or notify human operator to intervene) based on the output of a probabilistic classifier for the obstacle category. Suppose there is a loss for each action and the true obstacle category. For example, keep going when the obstacle is a car could incur a loss of -10000 while notifying the human operator costs -1. 


% For safe decision making, the probabilistic classifier is typically required to be (confidence) calibrated, i.e. among the times the classifier outputs 90\% confidence, the classification result should be correct with 90\% probability. Based on the confidence, the agent can decide which action to choose. If the confidence is high, the agent might opt for a more risky action (such as keep going); and if the confidence is low the agent might choose the safer action (which is notifying the human operator). 

% However, different types of mistakes can carry a different cost. For example, mis-classifying a car as drivable surface can lead to dangerous actions, while mis-classifying drivable surface as a car might not. Confidence calibration only measures if the classifier makes a mistake, but does not distinguish between different types of mistakes. To remedy this, distribution calibration (or strong calibration) has been proposed, but we will show that distribution calibration is difficult to achieve. To verify that a classifier approximately satisfies, we need a dataset with size that is exponentially large in the number of classification categories. 

% 

% Decision calibration is a general framework to understanding the types of guarantees each notion of calibration affords. We show that many existing calibration notions are equivalent to decision calibration, for a special set of decision tasks. 



% An example: suppose a healthcare provider is deciding whether a patient needs an invasive or expensive test. Based on current information, a prediction predicts the probability of different types of diseases. Suppose the healthcare provider decides to use the prediction to make decisions for all of its patient, it can compute the expected loss. 
















==> old.tex <==
% \begin{proof}[Proof of Lemma~\ref{lemma:radamacher_logistic}]
For $B^K_a$ we will prove with the covering number approach. 

We first recall the definition of the covering number. Given a set of functions $\Psi: \Zc \to \mathbb{R}$ and a set of samples $z_1, \cdots, z_N \in \Zc$, denote the $\epsilon$-covering number of $\Psi$ as $N_\infty(\epsilon, \Psi, N)$. In other words, there exists a set $\bfu_1, \bfu_2, \cdots \in \Rbb^N$ with cardinality $N_\infty(\epsilon, \Psi, N)$ such that $\forall \psi \in \Psi$ there exists some $\bfu_j$ and 
\begin{align*}
    \max_{n \in [N]} |\bfu_{jn} - \psi(z_n)| \leq \epsilon
\end{align*}
 
Because $\criticd(a)$ is the composition of linear functions with a softmax function, we first bound the covering number of linear functions with the following Lemma from \citep{zhang2002covering} Theorem 4. 
\begin{lemma}[Covering Number of Linear Functions] 
\label{lemma:linear_cover}
Let $\Phi_{\text{linear}}$ be the set of linear functions $\lbrace \bfz \mapsto \langle \bfw, \bfz \rangle, \lVert \bfz \rVert_\infty \leq 1, \lVert \bfw \rVert_1 \leq 1 \rbrace$ then there are constants $C_1, C_2 > 0$ such that 
\begin{align*}
   \log N_\infty(\epsilon, \Phi, N) \leq \frac{C_1}{\epsilon^2} \log \frac{n}{\epsilon} + C_2
\end{align*}
\end{lemma} 
To prove the covering number of $\criticd$ we prove the following composition theorem 
\begin{lemma}[Covering Number Composition]
\label{lemma:composition}
Let $\Phi^1, \cdots, \Phi^K$ be $K$ sets of functions $\Zc \to \Rbb$ and $\psi: \Rbb^K \to \Rbb$ be $L$-Lipschitz in the following sense: $\psi(\bfv + \delta \bfv) - \psi(\bfv) \leq L \lVert \delta \bfv \rVert_\infty, \forall \bfv, \delta \bfv \in \Rbb^K$. Then 
\begin{align*} 
\log N_\infty(L\epsilon, \psi(\Phi^1, \cdots, \Phi^K), N) \leq \sum_{k=1}^K \log N_\infty(\epsilon, \Phi^k, N)
\end{align*}
\end{lemma}
Finally what remains to show is that the softmax function is $L$-Lipschitz 
\begin{lemma}[Lipschitzness of Softmax]
\label{lemma:softmax_lipschitz}
Let $\psi: \Rbb^K \to \Rbb^K$ be the softmax function $\psi_k(v_1, \cdots, v_K) = \frac{e^{v_k}}{\sum_{k'} e^{v_{k'}}}$ then $\forall k, \psi_k$ is 2-Lipschitz with respect to the infinity norm, i.e. $\psi_k(\bfv + \delta \bfv) - \psi_k(\bfv) \leq 2 \lVert \delta \bfv \rVert_\infty, \forall \bfv, \delta \bfv \in \Rbb^K$. 
\end{lemma}

Given these Lemmas we are ready to complete the proof. 
\begin{align*}
   \log N_\infty(\epsilon, \criticd(a), N) & \leq K \log N_\infty(\epsilon/2, \Phi_{\text{linear}}, N) & \text{Lemma~\ref{lemma:softmax_lipschitz} and \ref{lemma:composition}} \\
   &\leq \frac{4KC_1}{\epsilon^2} \left( \log \frac{n}{\epsilon} + \log 2 \right)+ C_2 & \text{Lemma~\ref{lemma:linear_cover} and } \lVert \cdot \rVert_p \leq \lVert \cdot \rVert_q \text{ whenever } p \geq q \\
   &= \frac{KC_3}{\epsilon^2} \log \frac{n}{\epsilon} + C_4 & \text{New constants} 
\end{align*}
Also observe that $\lVert \cdot \rVert_\infty \leq \lVert \cdot \rVert_q$, $\forall q \in [1, \infty]$ we have
\begin{align*}
    N_q(\epsilon, \criticd(a), N) \leq N_\infty(\epsilon, \criticd(a), N)
\end{align*}
Finally we apply the covering number bound for Radamacher complexity to conclude that 
\begin{align*}
    \Rc(\criticd(a)) &\leq \inf_\epsilon \epsilon + \sqrt{\frac{2\log N_\infty(\epsilon, \criticd(a), N)}{N}} \\
    &=  \inf_\epsilon \epsilon + \sqrt{\frac{2KC_3}{\epsilon^2N}\log \frac{N}{\epsilon}+ \frac{C_4}{N}} \\
    &= O\left( \left(\frac{K}{N}\right)^{1/4}\log \frac{N}{K} \right) & \epsilon = (K/N)^{1/4} 
    %&\leq 12 \int_0^\infty \sqrt{\frac{\log N_\infty(\epsilon, \bar{B}^K_\alpha, n)}{n}} d\epsilon \\
    %&\leq O\left( \int_0^\infty \sqrt{\frac{K}{\epsilon^2n}\log \frac{n}{\epsilon}} d\epsilon \right) = O\left( \sqrt{\frac{K}{n}\log n}  \right) 
\end{align*}



Finally we prove the remaining Lemmas.
\begin{proof}[Proof of Lemma~\ref{lemma:softmax_lipschitz}] 
We first compute the derivative of $\psi_k$ as 
\begin{align*}
\frac{\partial}{\partial v_l} \psi_k(\bfv) = \left\lbrace \begin{array}{ll} \psi_k(\bfv) (1 - \psi_k(\bfv)) & k=l \\ -\psi_k (\bfv) \psi_l(\bfv) & k \neq l \end{array} \right.
\end{align*}
Then because $\psi$ is differentiable everywhere, choose any path $\bfu(t)$ such that $\bfu(0) = \bfv$ and $\bfu(1) = \bfv + \delta \bfv$ suppose $\lVert \delta \bfv \rVert_\infty \leq \epsilon$ we have 
\begin{align*}
    \psi_k(\bfv + \delta \bfv) - \psi_k(\bfv)
    %= \int_{t=0}^1 \psi_k'(\bfu(t))^T \bfu'(t) dt \leq \int_{t=0}^1 \psi_k'(\bfu(t))^T \lVert \bfu'(t) \right dt 
    &\leq \max_{\bfv'} \left(  \sum_l  \frac{\partial}{\partial v_l} \psi_k(\bfv') \delta \bfv_l \right)  \leq \epsilon \max_{\bfv'} \sum_l  \left\lvert \frac{\partial}{\partial v_l} \psi_k(\bfv') \right\rvert \\
    &= \epsilon \max_{\bfv'} \psi_k(\bfv')(1-\psi_k(\bfv') + \psi_l(\bfv')) \leq 2 \epsilon 
\end{align*}
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:composition}]
For any set of data points $\bfz = (z_1, \cdots, z_N) \in \Zc^N$, construct a $\epsilon$ cover for each $\Phi^k$ as $U^k = \lbrace \bfu^k_1, \bfu^k_2, \cdots \in \Rbb^N \rbrace$ such that $\forall \phi^k \in \Phi^K$ there exists some $\bfu^k_j$ and $\lVert \bfu^k_j - \phi^k(\bfz) \rVert \leq \epsilon$. 

Consider the product set $U^1 \otimes U^2 \cdots \otimes U^K$, and the set defined by 
\begin{align*}
    \lbrace \psi(\bfu^1, \cdots, \bfu^K), \bfu^1, \cdots, \bfu^K \in U^1 \otimes U^2 \cdots \otimes U^K \rbrace
\end{align*}
we claim that this is an $L\epsilon$-cover for $\psi(\Phi^1, \cdots, \Phi^K)$. This is because for any $\psi(\phi^1, \cdots, \phi^k) \in \psi(\Phi^1, \cdots, \Phi^K)$, consider the corresponding element $\bfu^k_{j_k} \in U^k$ such that $\lVert \bfu^k_j - \phi^k(\bfz) \rVert \leq \epsilon$ then 
\begin{align*}
    \left\lVert \psi(\bfu^1_{j_1}, \cdots,  \bfu^K_{j_K}) - \psi(\phi^1(\bfz), \cdots, \phi^K(\bfz) \right\rVert_\infty \leq \max_k \left\lVert \bfu^1_{j_k} - \phi^k(\bfz) \right\rVert_\infty \leq L\epsilon
\end{align*}
\end{proof} 

==> tables/satellite.tex <==
\begin{table*}
\begin{tabular}{llllllll}
\toprule
        &   & \textbf{Decision Loss} & \textbf{Decision Loss Gap} & \textbf{PCE} & \textbf{ECE} \\
Dataset & Calibration Method  &                            &         &                         &         &         &         \\
\midrule
\multirow{1}{*}{Satellite} & None  &        0.3510 $\pm$  0.0244 &            0.1000 $\pm$  0.0110 &                  0.0813 $\pm$  0.0145 &  0.0530 $\pm$  0.0169 \\
& Probabilistic (Posthoc) &        0.3458 $\pm$  0.0189 &            0.0888 $\pm$  0.0142 &                  0.0712 $\pm$  0.0250 &  0.0341 $\pm$  0.0118 \\
        & Point (Loss) &        0.3670 $\pm$  0.0236 &            \textbf{0.0798 $\pm$  0.0147} &                  \textbf{0.0524 $\pm$  0.0211} &  0.0441 $\pm$  0.0105 \\
        & Distribution(Posthoc)  &        0.3476 $\pm$  0.0226 &            0.0873 $\pm$  0.0182 &                  0.0615 $\pm$  0.0198 &  0.0379 $\pm$  0.0206 \\ 
\end{tabular}
\end{table*}

==> tables/uci.tex <==
\begin{table*}
\begin{tabular}{llllllll}
\toprule
        &   & \textbf{Decision Loss} & \textbf{Decision Loss Gap} & \textbf{PCE} & \textbf{ECE} \\
Dataset & Calibration Method  &                            &         &                         &         &         &         \\
\midrule
\multirow{1}{*}{Protein} & None &        0.5254 $\pm$  0.0082 &            0.0949 $\pm$  0.0051 &                  0.0927 $\pm$  0.0008 &  0.0399 $\pm$  0.0021 \\
& Probabilistic (Posthoc) &        0.5249 $\pm$  0.0084 &            0.0973 $\pm$  0.0061 &                  0.0952 $\pm$  0.0021 &  \textbf{0.0037 $\pm$  0.0010} \\
& Point (Posthoc) &         \textbf{0.5105 $\pm$  0.0073} &            \textbf{0.0285 $\pm$  0.0046} &  \textbf{0.0664 $\pm$ 0.0003} &  0.0065 $\pm$ 0.0008 \\
& Distribution (Posthoc) &        0.5706 $\pm$ 0.0140 &            0.0839 $\pm$  0.0114 &                  0.0936 $\pm$  0.0024 &  0.0528 $\pm$  0.0043 \\
\midrule
\multirow{1}{*}{Energy} & None &        0.1968 $\pm$  0.0337 &            0.0657 $\pm$  0.0264 &                  0.1295 $\pm$  0.0039 &  0.0977 $\pm$  0.0293 \\
&     Probabilistic (Posthoc) &   0.1875 $\pm$  0.0305 &            0.0381 $\pm$  0.0090 &                  0.0776 $\pm$  0.0162  &  \textbf{0.0066 $\pm$ 0.0027} \\
& Point (Posthoc) &        \textbf{0.1781 $\pm$  0.0266} &            \textbf{0.0223 $\pm$  0.0004} &                  \textbf{0.0725 $\pm$ 0.0109} &  \textbf{0.0066 $\pm$  0.0029} \\
& Distribution (Posthoc) &       0.2022 $\pm$  0.0265 &            0.0446 $\pm$  0.0060 &  0.0993 $\pm$  0.0095 &  0.0348 $\pm$  0.0057 \\
\midrule
\multirow{1}{*}{Naval} & None &        0.0519 $\pm$  0.0010 &            0.0648 $\pm$  0.0014 &                  0.2369 $\pm$  0.0050 &  0.1930 $\pm$  0.0079 \\
& Probabilistic (Loss)   &        0.0537 $\pm$  0.0016 &            0.0636 $\pm$  0.0014 &                  0.2277 $\pm$  0.0070 &  0.1769 $\pm$  0.0085 \\ 
        & Probabilistic (Posthoc)   &        0.0234 $\pm$  0.0041 &            0.0114 $\pm$  0.0027 &                  0.1762 $\pm$  0.0090 &  0.0072 $\pm$  0.0040 \\
        % & Point (Loss) &        0.0536 $\pm$ 0.0007 &            0.0658 $\pm$  0.0011 &                  0.2362 $\pm$  0.0049 &  0.1899 $\pm$ 0.0075 \\
        & Distribution (Posthoc) &        0.0362 $\pm$  0.0042 &            0.0351 $\pm$  0.0016 &                  0.2141 $\pm$ 0.0072 &  0.0566 $\pm$  0.0071 \\
\midrule
\multirow{1}{*}{Power-plant} & None &        0.1444 $\pm$  0.0025 &            0.0209 $\pm$  0.0029 &                  0.0851 $\pm$  0.0025 &  0.0204 $\pm$  0.0042 \\
& Probabilistic (Loss)   &        0.1445 $\pm$  0.0023 &            0.0178 $\pm$ 0.0009 &                  0.0823 $\pm$ 0.0039 &  0.0131 $\pm$  0.0039 \\
        & Probabilistic (Posthoc)   &        0.1438 $\pm$  0.0025 &            0.0203 $\pm$  0.0031 &                  0.0787 $\pm$  0.0026 &  0.0089 $\pm$  0.0020 \\
        % & Point (Loss) &        0.1460 $\pm$ 0.0020 &            0.0216 $\pm$  0.0024 &             0.0844 $\pm$  0.0028 &  0.0205 $\pm$ 0.0017  \\
        & Distribution (Posthoc) &        0.1535 $\pm$ 0.0069 &            0.0230 $\pm$  0.0045 &                  0.0952 $\pm$  0.0068 &  0.0163 $\pm$  0.0104 \\
\midrule
\multirow{1}{*}{Kin8nm} & None   &        0.1666 $\pm$  0.0038 &            0.0157 $\pm$  0.0022 &                  0.0819 $\pm$  0.0024 &  0.0140 $\pm$  0.0101 \\
& Probabilistic (Loss)   &        0.1648 $\pm$  0.0025 &            0.0162 $\pm$  0.0024 &                  0.0852 $\pm$  0.0063 &  0.0088 $\pm$  0.0030 \\
        & Probabilistic (Posthoc)   &        0.1664 $\pm$  0.0040 &            0.0150 $\pm$  0.0018 &                  0.0807 $\pm$  0.0030 &  0.0089 $\pm$ 0.0014 \\
%         & Point (Loss) &        0.1664 $\pm$  0.0033 &            0.0183 $\pm$  0.0030 &                0.0790 $\pm$  0.0007 &  0.0142 $\pm$  0.0079 \\
        & Distribution (Posthoc) &        0.1781 $\pm$  0.0063 &            0.0204 $\pm$  0.0034 &                  0.0903 $\pm$  0.0046 &  0.0255 $\pm$  0.0085 \\
% \midrule
% \multirow{1}{*}{Crime} & None  &        0.3561 $\pm$  0.0085 &            0.0743 $\pm$  0.0066 &                  0.0974 $\pm$  0.0075 & 0.0543 $\pm$  0.0118 \\
% & Probabilistic (Loss)   &        0.3554 $\pm$  0.0063 &            0.0814 $\pm$  0.0100 &                  0.0919 $\pm$ 0.0055 &  0.0426 $\pm$  0.0098 \\
%         & Probabilistic (Posthoc)   &        0.3517 $\pm$  0.0083 &            0.0554 $\pm$  0.0058 &                  0.0807 $\pm$  0.0065 &  0.0168 $\pm$  0.0083 \\
%         & Point (Loss) &        0.3575 $\pm$ 0.0044 &            0.0795 $\pm$  0.0090 &                  0.0921 $\pm$  0.0114 &  0.0492 $\pm$ 0.0099 \\
%         & Distribution(Posthoc) &        0.3861 $\pm$  0.0103 &            0.0628 $\pm$  0.0091 &                  0.1021 $\pm$  0.0095 &  0.0555 $\pm$  0.0180 \\

\bottomrule
\end{tabular}
\end{table*}


%& None  &        3.75 $\pm$  0.0200 &            0.0948 $\pm$  0.0050 &                  0.0926 $\pm$  0.0010 &  0.0397 $\pm$  0.0022 \\
%& Probabilistic (Loss)  &        3.75 $\pm$  0.0312 &            0.0962 $\pm$  0.0044 &                  0.0874 $\pm$  0.0018 &  0.0242 $\pm$  0.0062 \\
%        & Probabilistic (Posthoc)  &        3.77 $\pm$  0.0175 &            0.1221 $\pm$  0.0026 &                  0.1100 $\pm$  0.0003 &  \textbf{0.0025 $\pm$  0.0004} \\
        % & NLL + Posthoc Distribution Calibration &  3.06 &  0.0711 &            0.2195 &  0.0193 &                  0.1313 &  0.0015 &  0.0953 &  0.0058 \\
 %       & Point (Loss) & \textbf{3.73 $\pm$  0.0660} &            \textbf{0.0885  $\pm$ 0.0038} &                  \textbf{0.0841 $\pm$  0.0058} &  0.0370 $\pm$  0.0062 \\
